Verifying Pufferfish Privacy in Hidden Markov Models

Pufferfish is a Bayesian privacy framework for designing and analyzing privacy mechanisms. It refines differential privacy, the current gold standard in data privacy, by allowing explicit prior knowledge in privacy analysis. Through these privacy frameworks, a number of privacy mechanisms have been developed in literature. In practice, privacy mechanisms often need be modified or adjusted to specific applications. Their privacy risks have to be re-evaluated for different circumstances. Moreover, computing devices only approximate continuous noises through floating-point computation, which is discrete in nature. Privacy proofs can thus be complicated and prone to errors. Such tedious tasks can be burdensome to average data curators. In this paper, we propose an automatic verification technique for Pufferfish privacy. We use hidden Markov models to specify and analyze discretized Pufferfish privacy mechanisms. We show that the Pufferfish verification problem in hidden Markov models is NP-hard. Using Satisfiability Modulo Theories solvers, we propose an algorithm to analyze privacy requirements. We implement our algorithm in a prototypical tool called FAIER, and present several case studies. Surprisingly, our case studies show that na\"ive discretization of well-established privacy mechanisms often fail, witnessed by counterexamples generated by FAIER. In discretized \emph{Above Threshold}, we show that it results in absolutely no privacy. Finally, we compare our approach with testing based approach on several case studies, and show that our verification technique can be combined with testing based approach for the purpose of (i) efficiently certifying counterexamples and (ii) obtaining a better lower bound for the privacy budget $\epsilon$.

==> conclusions.tex <==
We have developed an automatic verification technique for
Pufferfish privacy.
We use HMMs to model privacy mechanisms
and analyze Pufferfish verification problems. A complexity lower
bound for the verification problem is shown to be NP-hard.
Nevertheless, the tool FAIER based on our automatic technique has analyzed several discrete privacy
mechanisms such as the truncated geometric mechanism, Noisy Max
and Above Threshold in the Pufferfish privacy
framework. Our analysis shows that na\"ive discretization can result
in privacy loss. In the worst case, the discrete Above Threshold
mechanism does not have any privacy guarantee at all.
We supply a comparison with
the state-of-the-art tool for differential privacy, and
propose to combine verification and testing for the purpose
of efficiently generating a precise lower
bound for the privacy budget $\epsilon$.
For future works, we plan to
optimize our work to deal with cases in differential privacy. Moreover,
it is interesting to investigate how to model and solve the verification problem
when continuous noise is applied.


==> evaluation.tex <==
We implement our verification algorithm (Algorithm~\ref{algorithm:pufferfish-check}) into the tool FAIER,
which is the pufferFish privAcy verifIER.
It is implemented both in \textbf{C++} and \textbf{Python} environment and
we performed all experiments on a Intel$\circledR$ Core i7-8750H
@ 2.20GHz CPU machine with 4 GB memory and 8 cores in the virtual machine.
All the examples in this paper have been verified by FAIER.
The inputs for our tool
include a hidden Markov model $H$ of the mechanism to be verified,
distributions pair ($\pi$,$\tau$) on states in $H$ for the databases distribution,
and a non-negative real number $c$ indicating
the privacy budget. Note that distributions can be represented as SMT formulae,
so that people can find out whether there exist $\pi$ and $\tau$ under certain constraints which violate privacy conditions.

There's also an input $k$ in Algorithm~\ref{algorithm:pufferfish-check} which specifies the length of observation
sequence to compare. If the privacy condition doesn't hold,
our tool will return a `SAT' answer and show the observation sequence, i.e, the counterexample, leading to the violation.
If there exist unknown parameters in the model, such as one infected with some disease of probability $p$, the values of them
will also be shown.
Otherwise, an `UNSAT' answer is returned meaning the privacy is preserved for this $k$, and if there exists a loop in the model, $k$ should continue to increase.
Our tool terminates if it finds a counterexample or $k$ is above a set value.
We summarize the experiment results in this paper for pufferfish privacy, as well as differential privacy in Table~\ref{table:experiment-results}, where
counterexample is the observation sequence that makes the mechanism violate privacy.

\begin{table*}[h]
\caption{Experiment results}
\label{table:experiment-results}
\begin{tabular}{p{3cm}<{\centering}|p{3cm}<{\centering}|p{2cm}<{\centering}|p{4cm}<{\centering}}
     \multirow{2}{*}{Mechanism} & \multirow{2}{*}{Privacy scenario} & \multicolumn{2}{c}{Result}  \\ \cline{3-4}
     & & Query answer & Counterexample  \\
      \hline
     \multirowcell{4}{Truncated \\$\frac{1}{2}$ -geometric \\Mechanism} & $\ln (2)$-differential privacy (Ex.~\ref{ex:hmm1}) & UNSAT & \\
     & $\ln (2)$-pufferfish privacy (Ex.~\ref{ex:hmm2})$^a$& SAT &$\tilde{2}$\\
     & $\ln (2)$-pufferfish privacy (Ex.~\ref{ex:hmm3})$^b$&
     SAT &$\tilde{0}$\\
     & $\ln (2)$-pufferfish privacy (Ex.~\ref{ex:hmm4})$^c$& UNSAT&\\
     \hline
     Naive Discrete Noisy Max (Algorithm~\ref{algorithm:noisy-max-naive})&
     $\ln (2)$-differential privacy (Ex.~\ref{ex:nnm})&SAT &$\bot,\tilde{0}$\\
     \hline
     \multirowcell{2}{Improved Discrete \\Noisy Max \\(Algorithm~\ref{algorithm:noisy-max})} &$\ln (2)$-pufferfish privacy (Ex.~\ref{ex:nm1})$^d$ & UNSAT(by REDLOG) &\\
     & $\ln (2)$-pufferfish privacy (Ex.~\ref{ex:nm2})$^e$& SAT &$\bot,\tilde{3}$\\
     \hline
     Above Threshold Algorithm (Algorithm~\ref{algorithm:above-threshold})& $4\ln (2)$-differential privacy & SAT &
     $\blank, 01, \bot,12,\bot,12$,$\bot$,$12$,$\bot$,$21,\top$\\
\end{tabular}
\end{table*}

The pufferfish privacy scenarios are listed below:

\renewcommand{\labelenumi}{\alph{enumi}.}
\begin{enumerate}
  \item with secrets a member contracting the disease or not.
  \item with secrets a member contracting the disease or not, knowing that the disease is highly contagious.
  \item with secrets contracting the disease is an independent event with fixed probability.
  \item with secrets a member contracting the disease A or not, knowing that
      the contraction of disease A, B and C is independent among individuals
  \item with secrets a member contracting the disease A or not, knowing that
      the disease A is highly contagious.
\end{enumerate}

Among the above mechanisms, Algorithm~\ref{algorithm:noisy-max-naive},\ref{algorithm:noisy-max},\ref{algorithm:above-threshold}
need our further investigation. We examine these algorithms carefully in the following sections.

%\subsubsection{Limitations}


==> logic.tex <==

\subsection{Syntax}

A \emph{state formula} $\phi$ is of the form
\[
  \top \ |\ 
  p \ |\ 
  \neg \phi \ |\ 
  \phi \wedge \phi \ |\ 
  \PJ{J} (\psi)
\]
where $\psi$ is a \emph{path formula} of the form
\[
  \X \psi \ |\ 
  \psi \until \psi \ |\ 
  \psi \until^{\leq n} \psi.
\]

\subsection{Semantics}

Let $M = (\Act, S, p, L)$ be an MDP, $s \in S$, and $\phi$ a PCTL
state formula. Define $M, s \models \phi$ as follows.

\[
\myPr{s}{K}{\phi} =
\Pr [ \{ \pi : K, \pi \models \psi \textmd{ with } \pi_0 = s \} ].
\]


\begin{eqnarray*}
  M, s \models \top\\
  M, s \models p  & \textmd{ if } &  p \in L(s)\\
  M, s \models \neg \phi  & \textmd{ if } &  M, s \not\models \phi\\
  M, s \models \phi \wedge \phi'
  & \textmd{ if } & M, s \models \phi \textmd{ and }
                    M, s \models \phi'\\
  M, s \models \PJ{J} \psi
  & \textmd{ if } &
  \myPr{s}{M_{\scheduler{S}}}{\psi} \in J
  \textmd{ for every scheduler } \scheduler{S}
\end{eqnarray*}

\begin{eqnarray*}
  K, \pi \models \X \psi
  & \textmd{ if } &
  K, \pi[1] \models \psi\\
  K, \pi \models \psi \until \psi'
  & \textmd{ if } &
  \textmd{there is a } j \geq 0 \textmd{ such that }
  K, \pi[j] \models \psi' \textmd{ and } \\
  & & K, \pi[k] \models \psi
      \textmd{ for every } 0 \leq k < j \\
  K, \pi \models \psi \until^{\leq n} \psi'
  & \textmd{ if } &
  \textmd{there is a } n \geq j \geq 0 \textmd{ such that }
  K, \pi[j] \models \psi' \textmd{ and } \\
  & & K, \pi[k] \models \psi \textmd{ for every } 0 \leq k < j
\end{eqnarray*}


Let $P = (M, \Obs, r)$ be a POMDP, $\info \in \info (S)$, and
$\phi$ a PCTL state formula. Define
\begin{eqnarray*}
  \myE{\info}{K}{\psi} = E_{\info} [K, \pi \models \psi
  \textmd{ with } \pi_0 = s].
\end{eqnarray*}
Define $P, \info \models \phi$ as follows.
\begin{eqnarray*}
  P, \info \models \top \\
  P, \info \models p & \textmd{ if } & \info \in \valueof{p}\\
  P, \info \models \neg \phi & \textmd{ if } & P, \info \not\models \phi\\
  P, \info \models \phi \wedge \phi' & \textmd{ if } &
       P, \info \models \phi \textmd{ and } P, \info \models \phi'\\
  P, \info \models \PJ{J} (\psi) & \textmd{ if } &
       \myE{\info}{M_{\scheduler{S}}}{\psi} \in J \\
  P, \info \models \dpriv{\epsilon}{\delta} (\psi) & \textmd{ if } &
       \myE{\info}{M_{\scheduler{S}}}{\psi} \leq e^{\epsilon}
       \myE{\info'}{M_{\scheduler{S}}}{\psi} + \delta \textmd{ and }\\
  &&   \myE{\info'}{M_{\scheduler{S}}}{\psi} \leq e^{\epsilon}
       \myE{\info}{M_{\scheduler{S}}}{\psi} + \delta \textmd{ for
     every } \info N \info'.
\end{eqnarray*}


==> preliminaries-pomdp.tex <==
A \emph{Markov decision process (MDP)} $M = (\Act, S, p, L)$ consists of
a finite set $\Act$ of \emph{actions}, a set $S$ of \emph{states}, a
\emph{labelling function} $L : S \rightarrow 2^{\AP}$, and 
a \emph{transition distribution} $p : \Act \times S \times S
\rightarrow \bbfRU$ such that $\sum_{t \in S} p (s, a, t) = 1$
for every $a \in \Act$ and $s \in S$. If the set of states is finite,
we say $M$ is a \emph{finite} MDP.

A \emph{partially observable Markov decision process (POMDP)} $P =
(M, \Obs, o)$ is a finite MDP $M = (\Act, S, p, L)$ with a finite set
$\Obs$ of \emph{observations} and an \emph{observation distribution} $o
: \Act  \times S \times \Obs \rightarrow \bbfRU$ such that $\sum_{\obs
  \in \Obs} o (a, s, \obs) = 1$ for every $a \in \Act$ and $s \in S$.
A POMDP models an MDP with incomplete information. The current state
of the underlying MDP is not known precisely. Rather, schedules are
made by observations and state distributions. 

Formally, let $\Info (S) = \{ \info \in S \rightarrow \bbfRU : \sum_{s \in
 S} \info (s) = 1 \}$ be the set of probability distributions on $S$. 
Consider an \emph{initial state distribution} $\info_0 \in \Info (S)$. A
\emph{history} $H_i$ up to time $i$ is a sequence $\info_0, a_1, \obs_1,
a_2, \obs_2, \ldots, a_{i-1}, \obs_{i-1}$. At time $i$, $H_i$ is the
only information available externally. If an action $a_i$ is chosen
at time $i$ based on $H_i$, the following steps are carried out
consecutively:
\begin{enumerate}
\item If the current state is $s_{i-1}$, the POMDP moves to the state
  $s_i$ with probability $p (s_{i-1}, a_i, s_i)$;
\item An observation $\obs_i$ is received with probability $o (a_i, s_i,
  \obs_i)$; and
\item The history $H_{i+1}$ becomes $H_i, a_i, \obs_i$.
\end{enumerate}
Note that histories do not contain states but the underlying MDP
updates its state as usual. Based on this formalization, we can now
define schedulers for POMDP. Let $\Xi$ be the set of histories. A
\emph{scheduler} $\sch{S} : \Xi \rightarrow \Act$ for the POMDP $P
= (M, \Obs, w)$ with $M = (\Act, S, p, L)$ is a function
from histories to actions. 

Interestingly, it is not necessary to keep
histories. For schedulers, it suffices to maintain the current state
distribution. Let $\info \in \Info (S)$ be a state distribution. Define
$T (\info, a, \obs) \in \Info (S)$ by
\begin{eqnarray}
  \Pr(\obs | \info, a) & = &
    \sum_{s, t \in S} \info (s) p (s, a, t) o (a, t, \obs)
\label{eqn:state-distribution-observation}
\\                             
  T (\info, a, \obs) (t) & = &
    \frac{\sum_{s \in S} \info (s) p (s, a, t) o (a, t, \obs)}
         {\Pr (\obs | \info, a)}.
\label{eqn:state-distribution-successor}
\end{eqnarray}
That is, $T (\info, a, \obs)$ is the posterior state distribution given
the prior state distribution $\info$, action $a$, and observation
$\obs$. Now recall that the initial state distribution $\info_0$ is
known. Let $\info_{i-1} \in \Info (S)$ be the state distribution at
time $i - 1$. Suppose a scheduler takes the action $a_{i}$ and
observes $\obs_{i}$ at time $i$. Then $\info_i = T (\info_{i-1}, a_i,
\obs_i)$ is the state distribution at time $i$. A
scheduler can then decide the next action $a_{i+1}$ by $\info_i$
accordingly. 

Let $R (s, a)$ be the reward for the state $s$ on the action
$a$, and $\overline{R} (s)$ be the reward for terminating at the state
$s$.\footnote{Observe that $R (s, a)$ is received when the MDP
\emph{leaves} $s$.} For $0 \leq \beta \leq 1$, the scheduler attaining
the maximal expected reward
\[
  E[\beta^T \overline{R} (s_T) + \sum_{i=0}^{T-1} \beta^i R(s_i, a_{i+1})]
\]
can be obtained by iteration. Let $L_{< \infty} (\Info (S))$ be the set of
bounded real-valued functions on $\Info (S)$. Consider
$\Upsilon : \Info (S) \times \Act \times L_{< \infty} (\Info (S)) \rightarrow
\bbfR$ defined by
\[
  \Upsilon (\info, a, f) = \sum_s \info (s) R (s, a) +
  \beta \sum_{\obs \in \Obs}
  \sum_{s, t \in S} \info (s) p (s, a, t) o (a, t, \obs) f (T (\info, a, \obs)).
\]
For $\info \in \Info (S)$, define
\begin{eqnarray}
  \overline{V}_{T} (\info) & = & \sum_s \info (s) \overline{R} (s)
\label{eqn:terminate-probability}
\\
  \overline{V}_{i} (\info) & = &
    \max_{a \in \Act} \{ \Upsilon (\info, a, \overline{V}_{i+1}) \} 
    \hspace{2em} (0 \leq i < T)
\label{eqn:max-probability}
\end{eqnarray}

It is more convenient to use matrices to simplify various
expressions. Without loss of generality, assume $S = \{ 1, 2, \ldots,
n \}$ when $|S| = n$. A state distribution $\info \in \Info (S)$ is
represented by the column vector $(\info (1), \info (2), \ldots, \info
(n))^T$  where $v^T$ is the transpose of the vector $v$.
For $a \in \Act$, let $P^a = [p_{ij}^a]_{|S|
  \times |S|}$ denote the transition matrix where $p_{ij}^a = p (i, a,
j)$. For $a \in \Act, \obs \in \Obs$, let $O^a (\obs) = [
o^a_{ij} ]_{|S| \times |S|}$ be the diagonal matrix where
\begin{eqnarray*}
  o^a_{ij} & = & \left\{
                 \begin{array}{ll}
                   o (a, i, \obs) & \textmd{ if } i = j\\
                   0 & \textmd{ otherwise}
                 \end{array}
                 \right.
\end{eqnarray*}
Let $e$ be the $n$-column vector whose entries are $1$.
Then $(\ref{eqn:state-distribution-observation})$ and
$(\ref{eqn:state-distribution-successor})$ rewrite to
\begin{eqnarray}
  \Pr (\obs | \info, a) & = & \info^T P^a O^a (\obs) e \\
  T (\info, a, \obs) & = & \frac{\info^T P^a O^a (\obs)}
                                {\Pr (\obs | \info, a)}
\end{eqnarray}
Similarly, let $R^a = (R (a, 1), R (a, 2), \ldots, R (a, n))^T$ be the
vector of rewards associated with the actcion
$a$. Equations~$(\ref{eqn:terminate-probability})$ and 
$(\ref{eqn:max-probability})$ rewrite to 
\begin{eqnarray}
  \overline{V}_{T} (\info) & = & \info^T \overline{R}\\
  \overline{V}_i (\info) & = &
        \max_{a \in \Act} \left\{ \info^T [
        R^a + 
        \beta \sum_{\obs \in \Obs}
          P^a O^a (\obs) \overline{V}_{i+1} ] \right\}
          \hspace{2em}(0 \leq i < T)
\end{eqnarray}

\hide{
\begin{eqnarray*}
  \overline{V}_{T} (\info) & = & \info^T \overline{R}\\
  \overline{V}_i (\info) & = &
        \max_{a \in \Act} \left\{ \info^T [
        R^a + 
        \beta \sum_{\obs \in \Obs} P^a O^a (\obs) \gamma^{l (\info, a,
                               \obs, i + 1)} ] \right\}\\
  l (\info, a, \obs, i) & = &
      \max_{\gamma \in \Gamma_{i}}
        \{ \info^T P^a O^a (\obs) \gamma \}
\end{eqnarray*}
}

==> subsampling.tex <==

\begin{algorithm}
  \begin{algorithmic}[1]
    \Function{SubsamplingMajority}{$d$, $f$}
    \Require{$d \in \{ R, B \}^n$, $f : \{ R, B \}^* \rightarrow \{ R,
      B \}$}
    \State{$q, m \leftarrow
            \frac{\epsilon}{64\ln (1/\delta)},
            \frac{\log (n/\delta)}{q^2}$}
    \State{Subsample $m$ data sets $\hat{d}_1, \hat{d}_2, \ldots,
      \hat{d}_m$ from $d$ where each row of $d$ is chosen with
      probability $q$}
    \label{algorithm:subsampling-majority-subsample}
    \State{$\mathit{count}_R, \mathit{count}_B \leftarrow
            | \{ i : f (\hat{d}_i) = R \} |,
            | \{ i : f (\hat{d}_i) = B \} |$}
    \label{algorithm:subsampling-majority-count}
    \State{$r \leftarrow | \mathit{count}_R - \mathit{count}_B | /
      (4mq) - 1$}
    \label{algorithm:subsampling-majority-difference}
    \If{${r} + \mathit{Lap}(\frac{1}{\epsilon}) > \ln (1/\delta)/\epsilon$}
    \label{algorithm:subsampling-majority-noise}
      \State{\textbf{if} $\mathit{count}_R \geq \mathit{count}_B$
             \textbf{then} \Return { $1$ } \textbf{else} \Return {$0$} }
      \label{algorithm:subsampling-majority-output}
    \Else
      \State{\Return {$\bot$}}
      \label{algorithm:subsampling-majority-mute}
    \EndIf
  \EndFunction
  \end{algorithmic}
  \caption{Subsampling Majority}
  \label{algorithm:subsampling-majority}
\end{algorithm}

\begin{figure}
  \centering
    \resizebox{\columnwidth}{!}{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node
      distance=2cm,node/.style={circle,draw}]

      \node[node] (rrr) at (-5,  1.5) { $rrr$ };
%      \node at (-4.4, 2) { $\vdots$ };
      \node[node] (rrb) at (-5.5,  0.55) { $rrb$ };
%      \node at (-4.4, .75) { $\vdots$ };
      \node[node] (rbb) at (-5.5, -0.55) { $rbb$ };
%      \node at (-4.4, -.5) { $\vdots$ };
      \node[node] (bbb) at (-5, -1.5) { $bbb$ };
%      \node at (-4.4, -1.75) { $\vdots$ };

      \node[node] (rmb0) at (-2.5,  1.5) { $m,0$ };
      \node at (-2.5, 0) { $\vdots$ };
      \node[node] (r0bm) at (-2.5, -1.5) { $0,m$ };

      \node[node] (Rm) at (0,  1.5) { $r_m$ };
      \node at (0, 0) { $\vdots$ };
      \node[node] (RM) at (0, -1.5) { $r_M$ };

      \node[node] (top) at (2.5,  0.75) { $\top$ };
      \node[node] (bot) at (2.5, -0.75) { $\bot$ };

      \node[node] (outR) at (5,  1.25) { $1$ };
      \node[node] (outB) at (5, .25) { $0$ };

      \path
      (rrr) edge node [above] { } (rmb0)
      (rrr) edge node [above] { } (r0bm)
      (rrb) edge node [above] { } (rmb0)
      (rrb) edge node [above] { } (r0bm)
      (rbb) edge node [above] { } (rmb0)
      (rbb) edge node [above] { } (r0bm)
      (bbb) edge node [above] { } (rmb0)
      (bbb) edge node [above] { } (r0bm)

      (rmb0) edge node [above] {} (RM)
      (r0bm) edge node [above] {} (RM)

      (Rm) edge node [above] {} (top)
      (Rm) edge node [above] {} (bot)
      (RM) edge node [above] {} (top)
      (RM) edge node [above] {} (bot)

      (top) edge (outR)
      (top) edge (outB)
      ;

      \end{tikzpicture}
    }
  \caption{Markov Chain for Subsampling Majority}
  \label{figure:subsampling-majority-markov-chain}
\end{figure}


==> wrongnoisymax.tex <==

\noindent
\textit{Example 7.3}
In Algorithm~\ref{algorithm:noisy-max}, the query \emph{index} with the
maximal noisy value is reported. This may appear unnatural. After all,
we are more interested in the maximal query result. It could be more
useful if the maximal noisy query result were reported.
Algorithm~\ref{algorithm:noisy-max-bad} shows the discrete noisy max
algorithm reporting the maximal noisy query result instead of the
query index.

In order to analyze the modified mechanism, we first construct its
formal model. For $n = 3$, the hidden Markov model for
Algorithm~\ref{algorithm:noisy-max-bad} is almost identical to
Figure~\ref{figure:hmm-noisy-max}. The only difference is the
observations and observation distributions for the bottom
states. Since noisy query results are reported, the set of
observations is $\{ \blank, \tilde{0}, \tilde{1}, \tilde{2} \}$. For
each bottom state, the maximal noisy query result of the state is
observed. For instance, $\tilde{2}$ is observed with probability $1$
at the state $0\underline{2}\underline{2}$.

In \emph{Example 7.1}, we have verified Figure~\ref{figure:hmm-noisy-max}
satisfied $\ln(2)$-Pufferfish privacy when contracting diseases is
independent among data entries. In addition, it also
satisfies $\ln(2)$-differential privacy on every pair of neighbouring states.
%With the same prior knowledge, our
%verification algorithm finds Algorithm~\ref{algorithm:noisy-max-bad}
%is not $\ln(2)$-Pufferfish private when $n = 3$.
%\todo{no neighboring states in Pufferfish privacy}
However, our tool finds Algorithm~\ref{algorithm:noisy-max-bad} is not
$\ln(2)$-differentially private. It checks all the pairs of neighbouring states and finds the
ratio of probabilities observing $\blank\tilde{0}$ on the neighboring states
$000$ and $110$ is larger than the multiplicative factor of $2$ within
2 seconds.
$\hfill\blacksquare$

\hide{
There's a variant version of Noisy Max, where it follows the usual settings
except at the last step the maximal
noisy result will be returned, as described in Algorithm \ref{algorithm:noisy-max-bad}.
This version has been considered to be wrong (not strictly proved) in the sense that it doesn't preserve differential privacy.
We can use an hidden Markov model to model this algorithm.
To be specific, the Markov chain part of this model is the same as in Algorithm \ref{algorithm:noisy-max}.
The difference is that the maximal value, instead of corresponding index, is observed in hidden Markov
model. For instance in the noisy-added state labeled $210$,
$2$ as the maximal value will be observed, while in the correct version of Noisy Max the corresponding index $1$ of $\tilde{v}_1$ is observed.
Using our Pufferfish checking algorithm, we can easily check whether
Algorithm \ref{algorithm:noisy-max-bad} satisfies differential privacy.
One important thing to be noted is that, in some cases where $n$ is small,
differential privacy is still preserved.
For instance our implementation returns ``unsat'' when $n=5$, meaning that
$\ln(2)$-differential privacy is still preserved under this case.
This result doesn't violate the general consideration of the algorithm;
instead, it shows that specific privacy scenarios can be verified using our algorithm.
}

\begin{algorithm}
  \begin{algorithmic}[1]
    \Require{$0 \leq v_1, v_2, \ldots, v_n \leq 2$}
    \Ensure{The maximal $v_r$ among $v_1, v_2, \ldots, v_n$}
    \Function{NoisyMax}{$v_1, v_2, \ldots, v_n$}
      \State{$M \leftarrow -1$}
      \For{each $v_i$}
        \Match{$v_i$}
        \Comment{apply $\frac{1}{2}$-geometric mechanism}
          \lCase{$0$}
                {$\tilde{v}_i \leftarrow 0, 1, 2$ with probability
                 $\frac{2}{3}, \frac{1}{6}, \frac{1}{6}$}
          \lCase{$1$}
                {$\tilde{v}_i \leftarrow 0, 1, 2$ with probability
                 $\frac{1}{3}, \frac{1}{3}, \frac{1}{3}$}
          \lCase{$2$}
                {$\tilde{v}_i \leftarrow 0, 1, 2$ with probability
                 $\frac{1}{6}, \frac{1}{6}, \frac{2}{3}$}
        \EndMatch
        \If{$M < \tilde{v}_i$}
          \State{$M \leftarrow \tilde{v}_i$}
        \EndIf
      \EndFor
      \State{\Return {$M$} }
    \EndFunction
  \end{algorithmic}
  \caption{Wrong Version of Noisy Max}
  \label{algorithm:noisy-max-bad}
\end{algorithm}

In Algorithm~\ref{algorithm:noisy-max}, we have considered
multiple queries with the same maximal noisy value. If
more than one query have the same maximal noisy value, one of their
indices is reported uniformly randomly. A na\"ive adoption of the
standard noisy max algorithm could simply return an index
deterministically. It would not have the same privacy guarantee.

\noindent
\textit{Example 7.4}
Algorithm~\ref{algorithm:noisy-max-naive} shows a na\"ive
discretization of the standard noisy max algorithm. The algorithm
simply updates the maximal noisy query result $M$ and the index $r$
when a larger noisy result is encountered. Subsequently, the na\"ive
algorithm reports the index of the first query with the maximal noisy
result. At the first glance, the na\"ive discretization does not appear
harmful. It is not so after our formal analysis.

\begin{algorithm}
  \begin{algorithmic}[1]
    \Require{$0 \leq v_1, v_2, \ldots, v_n \leq 2$}
    \Ensure{The maximal $v_r$ among $v_1, v_2, \ldots, v_n$}
    \Function{NoisyMax}{$v_1, v_2, \ldots, v_n$}
      \State{$M, r \leftarrow -1, 0$}
      \For{each $v_i$}
        \Match{$v_i$}
        \Comment{apply $\frac{1}{2}$-geometric mechanism}
          \lCase{$0$}
                {$\tilde{v}_i \leftarrow 0, 1, 2$ with probability
                 $\frac{2}{3}, \frac{1}{6}, \frac{1}{6}$}
          \lCase{$1$}
                {$\tilde{v}_i \leftarrow 0, 1, 2$ with probability
                 $\frac{1}{3}, \frac{1}{3}, \frac{1}{3}$}
          \lCase{$2$}
                {$\tilde{v}_i \leftarrow 0, 1, 2$ with probability
                 $\frac{1}{6}, \frac{1}{6}, \frac{2}{3}$}
        \EndMatch
        \If{$M < \tilde{v}_i$}
          \State{$M, r \leftarrow \tilde{v}_i, i$}
        \EndIf
      \EndFor
      \State{\Return {$r$} }
    \EndFunction
  \end{algorithmic}
  \caption{Naive Discrete Noisy Max}
  \label{algorithm:noisy-max-naive}
\end{algorithm}

%Assume disease contraction is independent for each data entries.
%Algorithm~\ref{algorithm:noisy-max} is verified to satisfy
%$\ln(2)$-Pufferfish privacy previously.
We perform the same analysis
on Algorithm~\ref{algorithm:noisy-max-naive} using our verification
algorithm. Interestingly, Algorithm~\ref{algorithm:pufferfish-check}
shows that the na\"ive discretization is not $\ln(2)$-differentially
private, with a ratio of probabilities observing $\blank\tilde{0}$ larger
than 2 on a pair of neighboring states.
It is not sufficient to replace continuous noises with
discrete noises. Additional steps are required to preserve privacy.
An inexperienced mechanism designer may na\"ively discretize
the standard noisy max algorithm and put privacy at risk. Designing
privacy mechanisms can be very tricky indeed.
